Beyond Neyman-Pearson: e-values enable hypothesis testing with a data-driven alpha

A standard practice in statistical hypothesis testing is to mention the p-value alongside the accept/reject decision. We show the advantages of mentioning an e-value instead. With p-values, it is not clear how to use an extreme observation (e.g. p $\ll \alpha$) for getting better frequentist decisions. With e-values it is straightforward, since they provide Type-I risk control in a generalized Neyman-Pearson setting with the decision task (a general loss function) determined post-hoc, after observation of the data -- thereby providing a handle on `roving $\alpha$'s'. When Type-II risks are taken into consideration, the only admissible decision rules in the post-hoc setting turn out to be e-value-based. Similarly, if the loss incurred when specifying a faulty confidence interval is not fixed in advance, standard confidence intervals and distributions may fail whereas e-confidence sets and e-posteriors still provide valid risk guarantees. Sufficiently powerful e-values have by now been developed for a range of classical testing problems. We discuss the main challenges for wider development and deployment.

==> declarations.tex <==
\usepackage{epsf}
\usepackage{verbatim}
\usepackage{makeidx}
%\usepackage{psfrag}
\usepackage{graphicx}
%\usepackage{psfig}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{latexsym}
\usepackage{amsbsy}
\usepackage{epsfig}


\setlength{\textwidth}{15.5 cm}
\setlength{\textheight}{22.4 cm}
\setlength{\topmargin}{-1.3 cm}
\setlength{\hoffset}{-1.4cm}
\setlength{\evensidemargin}{1.4 cm}
\setlength{\oddsidemargin}{1.4cm}



\newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{fact}{Fact}
\newtheorem{condition}{Condition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{cor}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{sublemma}{Sublemma}
\newtheorem{proposition}{Proposition}
\newtheorem{question}{Question}
\newtheorem{definition}{Definition}



\newcommand{\commentout}[1]{}
\newcommand{\prs}{\par}
\newenvironment{shortproof}{\setlength{\parindent}{0mm}
{\setlength{\parskip}{0mm}
\raggedright\noindent\bf Proof}:}{$\Box$}
\newenvironment{proof}{\noindent{\bf Proof}:}{\mbox{$\Box$}
\prs\vspace{3mm}\prs}
\newenvironment{stage}
{\setlength{\parindent}{0mm}\setlength{\parskip}{1mm}\prs
\noindent{\bf stage} $n$:\prs

\addtolength{\leftskip}{5mm}}{\prs\addtolength{\leftskip}
{-5mm}\noindent {\bf end of stage} $n$\prs}
\newcommand{\emptyline}{\vspace{\baselineskip}}
\newcommand{\halfemptyline}{\vspace{.25cm}}

\newcounter{repeatproba}
\newcounter{repeatprobb}
\newcounter{repeatprobc}
\newcounter{lemmastronglawcounter}
\newcounter{snavel}

\newcounter{myenumeratecounter}
\newenvironment{myenumerate}{\begin{list}
{\arabic{myenumeratecounter}.}
{
\usecounter{myenumeratecounter}
\setlength{\itemsep}{0.0 cm}
}
}
{\end{list}}

\newtheorem{examplehidden}{Example}
\newenvironment{example}{
\begin{examplehidden}
\em
}
{\end{examplehidden}}

\newcommand{\ownbox}[2]{
\noindent \ \vspace{\baselineskip} \\
\noindent
\fbox{\hspace*{\ownleftboxwidth} \parbox{\ownboxwidth}{\
\\
{\bf #1
} \\ \noindent #2 }\hspace*{\ownrightboxwidth}
} \ \vspace{\baselineskip} \\}

\newenvironment{ownquote}
               {
\list{}{\rightmargin\leftmargin}%
                \small \item[]}
               {\endlist}

%\newenvironment{examplea}{
%\setcounter{examplehidden}{0}
%\begin{examplehidden}[continued]
%\em
%}
%{\end{examplehidden}}
%\newenvironment{exampleb}{
%%\setcounter{examplehidden}{1}
%\begin{examplehidden}[continued]
%\em
%}
%{\end{examplehidden}}


% SAFESTATS THINGS

\newcommand{\G}{\ensuremath{\langle G \rangle}}
\newcommand{\E}[3]{\ensuremath{\text{\rm E}_{#1  #2}[#3]}}
\newcommand{\weak}[1]{\ensuremath{\langle #1 \rangle_{\text{\rm weak}}}}
\newcommand{\strong}[1]{\ensuremath{\langle #1 \rangle_{\text{\rm strong}}}}
\newcommand{\super}[1]{\ensuremath{\langle #1 \rangle_{\text{\rm super}}}}
\newcommand{\strongsuper}[1]{\ensuremath{\langle#1\rangle_{\text{\rm strong,super}}}}
\newcommand{\determines}{\ensuremath{\rightsquigarrow}}
\newcommand{\hyp}{\ensuremath{H}}
\newcommand{\Pbayes}{\ensuremath{P}_{\text{B}}}
\newcommand{\pval}{\ensuremath{{\tt pval}}}
\newcommand{\qval}{\ensuremath{{\tt qval}}}
\newcommand{\pcrit}{\ensuremath{{\tt p}_0}}


\newcommand{\dnl}[1]{{\ensuremath{\bar{\text{\rm d}}_{#1}}}}
\newcommand{\dul}[1]{{\ensuremath{{\text{\rm d}}_{#1}}}}
\newcommand{\entropyrenyi}[1]{{\ensuremath{{\text{\rm H}}_{#1}}}}
\newcommand{\bhellinger}[1]{{\ensuremath{{\text{\rm He}}_{#1}}}}
\newcommand{\squaredhellinger}[1]{{\ensuremath{{\text{\rm He}}^2_{#1}}}}
\newcommand{\af}{{\ensuremath{{\text{A}}}}}
\newcommand{\resolvability}{{\text{\sc RES}}}
\newcommand{\cesarorisk}{{\overline{\text{\sc RISK}}}}



\newcommand{\puniv}{\ensuremath{\bar{P}}}
\newcommand{\lunivtop}{\ensuremath{\bar{L}_{\text{\rm top}}}}
\newcommand{\punivtop}{\ensuremath{\bar{P}_{\text{\rm top}}}}
\newcommand{\funivtop}{\ensuremath{\bar{f}_{\text{\rm top}}}}
\newcommand{\funivrsy}{\ensuremath{\bar{f}_{\text{\rm RSY}}}}
%\newcommand{\punivsemibayes}{\ensuremath{\bar{P}_{\text{\rm semi-Bayes}}}}
%\newcommand{\funivsemibayes}{\ensuremath{\bar{f}_{\text{\rm semi-Bayes}}}}
%\newcommand{\lunivsemibayes}{\ensuremath{\bar{L}_{\text{\rm semi-Bayes}}}}
\newcommand{\lunivsemitop}{\ensuremath{\bar{L}_{\text{\rm semi-top}}}}
\newcommand{\punivsemitop}{\ensuremath{\bar{P}_{\text{\rm semi-top}}}}
\newcommand{\lunivlbayes}{\ensuremath{\bar{L}_{\text{\rm lucky-Jeffreys}}}}
\newcommand{\punivlbayes}{\ensuremath{\bar{P}_{\text{\rm lucky-Jeffreys}}}}
\newcommand{\punivsolomonoff}{\ensuremath{\bar{P}_{\text{\rm Solomonoff}}}}
\newcommand{\funivlbayes}{\ensuremath{\bar{f}_{\text{\rm lucky-Jeffreys}}}}
\newcommand{\funivkernel}{\ensuremath{\bar{f}_{\kernel}}}
\newcommand{\lunivlaplace}{\ensuremath{\bar{L}_{\text{\rm Laplace}}}}
\newcommand{\punivlaplace}{\ensuremath{\bar{P}_{\text{\rm Laplace}}}}
\newcommand{\quniv}{\ensuremath{\bar{Q}}}
\newcommand{\punivplugin}{\ensuremath{\bar{P}_{\text{\rm plug-in}}}}
\newcommand{\punivtp}{\ensuremath{\bar{P}_{\text{\rm 2-p}}}}
\newcommand{\punivcrude}{\ensuremath{\bar{P}_{\text{\rm crude}}}}
\newcommand{\punivref}{\ensuremath{\bar{P}_{\text{\rm refined}}}}
\newcommand{\punivseq}{\ensuremath{\bar{P}_{\text{\rm seq}}}}
\newcommand{\punivseqn}[1]{\ensuremath{\bar{P}_{\text{\rm seq},#1}}}
\newcommand{\punivopt}{\ensuremath{\bar{P}_{\text{\rm opt}}}}
\newcommand{\punivmodsel}{\ensuremath{\bar{P}_{\text{\rm modsel}}}}
\newcommand{\punivmdlaic}{\ensuremath{\bar{P}_{\text{\rm mdl-aic}}}}
\newcommand{\funivmodsel}{\ensuremath{\bar{P}_{\text{\rm modsel}}}}
\newcommand{\optprior}{\ensuremath{{\prior}_{\text{\rm opt}}}}
\newcommand{\punivmeta}{\ensuremath{\bar{P}_{\text{\rm meta}}}}
\newcommand{\funivmeta}{\ensuremath{\bar{f}_{\text{\rm meta}}}}
\newcommand{\funiv}{\ensuremath{\bar{f}}}
\newcommand{\lunivhy}{\ensuremath{\bar{L}_{\text{\rm HY}}}}
\newcommand{\funivlb}{\ensuremath{\bar{f}_{\text{\rm LB}}}}
\newcommand{\punivlb}{\ensuremath{\bar{P}_{\text{\rm LB}}}}
\newcommand{\lunivlb}{\ensuremath{\bar{L}_{\text{\rm LB}}}}
\newcommand{\punivrnml}{\ensuremath{\bar{P}_{\text{\rm Rnml}}}}
\newcommand{\punivcnmla}{\ensuremath{\bar{P}_{\text{\rm Cnml-1}}}}
\newcommand{\punivcnmlb}{\ensuremath{\bar{P}_{\text{\rm Cnml-2}}}}
\newcommand{\punivlnmla}{\ensuremath{\bar{P}_{\text{\rm Lnml-1}}}}
\newcommand{\punivlnmlb}{\ensuremath{\bar{P}_{\text{\rm Lnml-2}}}}
\newcommand{\funivcnmla}{\ensuremath{\bar{f}_{\text{\rm Cnml-1}}}}
\newcommand{\funivcnmlb}{\ensuremath{\bar{f}_{\text{\rm Cnml-2}}}}
\newcommand{\funivlnmla}{\ensuremath{\bar{f}_{\text{\rm Lnml-1}}}}
\newcommand{\funivlnmlb}{\ensuremath{\bar{f}_{\text{\rm Lnml-2}}}}
%\newcommand{\punivnmap}{\ensuremath{\bar{P}_{\text{\rm nmap}}}}
\newcommand{\punivnml}{\ensuremath{\bar{P}_{\text{\rm nml}}}}
\newcommand{\funivnml}{\ensuremath{\bar{f}_{\text{\rm nml}}}}
\newcommand{\funivbayes}{\ensuremath{\bar{f}_{\text{\rm Bayes}}}}
\newcommand{\funivrnml}{\ensuremath{\bar{f}_{\text{\rm Rnml}}}}
\newcommand{\funivrrnml}{\ensuremath{\bar{f}_{\text{\rm RRnml}}}}
\newcommand{\punivnmln}[1]{\ensuremath{\bar{P}_{\text{\rm nml},#1}}}
\newcommand{\punivbayes}{\ensuremath{\bar{P}_{\text{\rm Bayes}}}}
\newcommand{\punivpreq}{\ensuremath{\bar{P}_{\text{\rm preq}}}}
\newcommand{\punivcesaro}{\ensuremath{\bar{P}_{\text{\rm Cesaro}}}}
\newcommand{\punivcesarb}{\ensuremath{\bar{P}_{\text{\rm Cesaro}\mid n-1}}}
\newcommand{\punivsmml}{\ensuremath{\bar{P}_{\text{\rm smml}}}}
\newcommand{\punivjmod}{\ensuremath{\bar{P}_{n,\text{\rm Jef}^+}}}
\newcommand{\punivjeffreys}{\ensuremath{\bar{P}_{\text{\rm Jeffreys}}}}
\newcommand{\funivjeffreys}{\ensuremath{\bar{f}_{\text{\rm Jeffreys}}}}
\newcommand{\funivlaplace}{\ensuremath{\bar{f}_{\text{\sc u}}}}
\newcommand{\luniv}{\ensuremath{\bar{L}}}
\newcommand{\lunivtp}{\ensuremath{\bar{L}_{\text{\rm 2-p}}}}
\newcommand{\lunivtpopt}{\ensuremath{\bar{L}_{\text{\rm 2-p, opt}}}}
\newcommand{\lunivatp}{\ensuremath{\bar{L}_{\alpha 2 \text{\rm -p}}}}
\newcommand{\punivatp}{\ensuremath{\bar{P}_{\alpha 2 \text{\rm -p}}}}
\newcommand{\lunivtpcond}{\ensuremath{\bar{L}_{\text{\rm cond-2-p}}}}
\newcommand{\lunivnml}{\ensuremath{\bar{L}_{\text{\rm nml}}}}
\newcommand{\lunivbayes}{\ensuremath{\bar{L}_{\text{\rm Bayes}}}}
\newcommand{\lunivsmml}{\ensuremath{\bar{L}_{\text{\rm smml}}}}
\newcommand{\kc}{\ensuremath{{K}}}
\newcommand{\lunivkc}{\ensuremath{\bar{L}_{\text{\rm Kolmogorov}}}}
\newcommand{\lunivkcN}[1]{\ensuremath{\bar{L}_{\text{\rm Kolmogorov},#1}}}
\newcommand{\punivkc}{\ensuremath{\bar{P}_{\text{\rm Kolmogorov}}}}

\newcommand{\ctp}{\ensuremath{\const_{\text{\rm 2-p}}}}
\newcommand{\cnml}{\ensuremath{\const_{\text{\rm nml}}}}
\newcommand{\cbayes}{\ensuremath{\const_{\text{\rm Bayes}}}}


\newcommand{\cA}{\ensuremath{\mathcal A}}
\newcommand{\cB}{\ensuremath{\mathcal B}}
\newcommand{\cC}{\ensuremath{\mathcal C}}
\newcommand{\cD}{\ensuremath{\mathcal D}}
\newcommand{\cE}{\ensuremath{\mathcal E}}
\newcommand{\cF}{\ensuremath{\mathcal F}}
\newcommand{\cG}{\ensuremath{\mathcal G}}
\newcommand{\cH}{\ensuremath{\mathcal H}}
\newcommand{\cI}{\ensuremath{\mathcal I}}
\newcommand{\cJ}{\ensuremath{\mathcal J}}
\newcommand{\cK}{\ensuremath{\mathcal K}}
\newcommand{\cL}{\ensuremath{\mathcal L}}
\newcommand{\cM}{\ensuremath{\mathcal M}}
\newcommand{\cN}{\ensuremath{\mathcal N}}
\newcommand{\cO}{\ensuremath{\mathcal O}}
\newcommand{\cP}{\ensuremath{\mathcal P}}
\newcommand{\cQ}{\ensuremath{\mathcal Q}}
\newcommand{\cR}{\ensuremath{\mathcal R}}
\newcommand{\cS}{\ensuremath{\mathcal S}}
\newcommand{\cT}{\ensuremath{\mathcal T}}
\newcommand{\cU}{\ensuremath{\mathcal U}}
\newcommand{\cV}{\ensuremath{\mathcal V}}
\newcommand{\cW}{\ensuremath{\mathcal W}}
\newcommand{\cX}{\ensuremath{\mathcal X}}
\newcommand{\cY}{\ensuremath{\mathcal Y}}
\newcommand{\cZ}{\ensuremath{\mathcal Z}}

% CONVENTIONS:

% 1. NOTATIONAL SYSTEM

% greek capitals for parameter spaces (including \Delta for unit simplex)
% small greek letters for points in parameter spaces 
%               (eg \freq, still needed in chapter 1)

% ordinary caps (sometimes in \rm) 
% for mathematical function(al)s, operations such as
% entropy, KL divergence, expectation etc.

% ordinary (no caps) letters for functions:
% f : density
% g,h : ordinary function

% D : data
% H : simple hypothesis
% H : function in role of simple hypothesis, in chapter 1 and
% introduction (formally different from simple hypothesis, but
% impossible to disentangle)

% Models: \cal (such as \M, \Bernoulli)
% General hypotheses (can be both sets or singleton sets) :
% {\cal H}
% sample spaces: calligraphic

% L(x) length of binary string C(x)
% l(x), l_x : length of x itself

% other sets: calligraphic

% \circ, or _0 for open sets


% m: maxoutcome in a set
% l: dimensionality sample space
% k: dimensionality parameter space

% dimensionality of parameter, model/index of parameter/model
% \M^{(5)} used for 5-dimensional model; \Theta^{(5)} for 5-dimensional
% parameter space; \theta^{(5)} for element of such a parameter space
% \M_1, \M_2 used to index different models 
% if we do not want to be specific about 
% their number of parameters; similar for \Theta_1, \Theta_2, ...
%
% \theta_1, ..., \theta_k usually denotes COMPONENT of vector \theta.
% also sometimes used to index different vectors \theta -> try to avoid this!
% (avoided it nearly everywhere - use \theta^\circ, \theta' instead. 
% This also nicely fits in with use of \hat{\theta}, \theta^*

% when I need to index ML estimator or two-part estimator by sample size,
% use \twop{\theta}_{(n)}, \hat{\theta}_{(n)}
%


% Sequence/Vector notation of sample: 
% write D = x^n =  (x_1, \ldots, x_n) met haakjes; altijd haakjes gebruiken (vector interpretatie)
% behalve als je direct over coderen praat, of over begin van oneindige sequenties

%2. NOTATION IN PARTICULAR

% \Theta_\M is really needed in chapter 2



% general mathematical operations

\newcommand{\myargmax}[1]{\ensuremath{\underset{#1}{\ \arg \max \ }}}
\newcommand{\myargmin}[1]{\ensuremath{\underset{#1}{\ \arg \min \ }}}
\newcommand{\isbydefinition}{\ensuremath{{:=}}}
%pdg: \isbydefinition changed 15-8-03. Was '\equiv'
\newcommand{\stsum}{\sum_{i=1}^n}
\newcommand{\transpose}{\ensuremath{{\text{\sc T}}}}
\newcommand{\indicator}{\ensuremath{{\mathbf 1}}}


\newcommand{\distance}{\ensuremath{{d}}}


\newcommand{\freq}{\ensuremath \gamma}
\newcommand{\remainder}{\ensuremath R}
\newcommand{\constant}{\ensuremath{K}}
\newcommand{\const}{\ensuremath{c}}

% SETS AND THEIR ELEMENTS 

% SETS 1: general sets

\newcommand{\reals}{{\mathbb R}}
\newcommand{\booleans}{{\mathbb B}}
\newcommand{\integers}{{\mathbb Z}}
\newcommand{\naturals}{{\mathbb N}}
\newcommand{\simplexN}[1]{\ensuremath{\Delta}^{(#1)}}

% TOPOLOGY

\newcommand{\closure}{\ensuremath{\mathrm{cl \ }}}
\newcommand{\interior}{\ensuremath{\mathrm{int \ }}}
\newcommand{\ball}{\ensuremath{B}}


% SETS 2: Outcomes and Sample Spaces.

\newcommand{\justaset}{\ensuremath {\mathcal U}}
\newcommand{\justanevent}{\ensuremath {\mathcal E}}
\newcommand{\justasymbol}{\ensuremath {s}}
% \justasymbol denoted to use an element of sample space in contexts
% where x is already used (ie Does s occur in sample x_1, ..., x_n ?)

% we use l for dimensionality of sample space, k for dimensionality of
% parameter space, and m for dimensionality of general space, if we do not
% want to commit to an interpretation (eg beginning of chapter 2)


\newcommand{\data}{\ensuremath D}
\newcommand{\dataalphabet}{\ensuremath \mathcal A}
\newcommand{\samplespace}{\ensuremath {{\mathcal X}}}
%peter 22-7-03: note Xspace and samplespace now the same symbol!
\newcommand{\xspace}{\ensuremath {{\mathcal X}}}
\newcommand{\yspace}{\ensuremath {{\mathcal Y}}}
\newcommand{\zspace}{\ensuremath {{\mathcal Z}}}
\newcommand{\outcomex}{\ensuremath x}
\newcommand{\outcomey}{\ensuremath y}
\newcommand{\bogus}{\ensuremath \Box}
\newcommand{\maxoutcome}{\ensuremath m}
\newcommand{\region}{\ensuremath{{\mathbf R}}}


%SETS AND ELEMENTS 3: estimators/hypotheses/parameters

%\newcommand{\mldim}[1]{\ensuremath{\hat{\theta}_{#1}}}
\newcommand{\mlN}[1]{\ensuremath{\hat{\theta}^{(#1)}}}
\newcommand{\ml}{\ensuremath \hat{\theta}}
\newcommand{\mapest}{\ensuremath \breve{\theta}}
\newcommand{\param}{\ensuremath {\theta}}
\newcommand{\paramN}[1]{\ensuremath {\theta}^{(#1)}}
\newcommand{\meanest}{\ensuremath \bar{\theta}}
\newcommand{\truepar}{\ensuremath \theta^*}
\newcommand{\trueprob}{\ensuremath \prob^*}

\newcommand{\twop}[1]{\ensuremath{{\ddot{#1}}}} 
\newcommand{\twopN}[2]{\ensuremath{{\ddot{#1}^{(#2)}}}}
%\newcommand{\trml}{\hat{\ddot{\theta}}}
\newcommand{\mcparam}[1]{\ensuremath{\theta_{[1|#1]}}}
\newcommand{\mcmlparam}[1]{\ensuremath{\hat{\theta}_{[1|#1]}}}
\newcommand{\mctrueparam}[1]{\ensuremath{{\theta}^*_{[1|#1]}}}
\newcommand{\mcmlparamb}[2]{\ensuremath{\hat{\theta}_{[#1|#2]}}}
\newcommand{\utm}{\ensuremath{\text{\sc{ul}}}}

\newcommand{\phyp}{\ensuremath {H}}
\newcommand{\ghyp}{\ensuremath {\mathcal H}}
%phyp = point hypothesis
%ghyp = general (point or compound) hypothesis
\newcommand{\hfun}{\ensuremath {h}}

%SETS AND ELEMENTS 4: parameter SETS

%\newcommand{\parasetN}[1]{\ensuremath{\Theta_{#1}}}
\newcommand{\parasetN}[1]{\ensuremath{\Theta^{(#1)}}}
\newcommand{\paraset}{\ensuremath{\Theta}}
%\newcommand{\trparaset}[2]{\ensuremath{{\ddot{\Theta}^{#2}_{#1}}}}
\newcommand{\twopparaset}[2]{\ensuremath{{\ddot{\Theta}^{(#1)}_{#2}}}}

% codes and codelengths

\newcommand{\clengthnr}{\ensuremath{l}}

\newcommand{\lunif}{\ensuremath{L_{U}}}
\newcommand{\punif}{\ensuremath{P_{U}}}
\newcommand{\Lint}{\ensuremath{L_{\naturals}}}
\newcommand{\punivint}{\ensuremath{\bar{P}_{\naturals}}}
\newcommand{\indexcode}{\ensuremath C_{\text{index}}}
\newcommand{\shannoncode}{\ensuremath C_{\text{Shannon}}}
\newcommand{\Lindex}{\ensuremath L_{\text{index}}}
\newcommand{\Lshannon}{\ensuremath L_{\text{Shannon}}}
\newcommand{\prefixlengths}{\ensuremath{\mathcal{L}}}
\newcommand{\code}{\ensuremath C}
\newcommand{\CN}[1]{\ensuremath C^{(#1)}}
\newcommand{\codelength}{\ensuremath{L}}
\newcommand{\codelengths}{\ensuremath{\mathcal{L}}}
\newcommand{\regret}{\ensuremath{\mathcal R}}

% functions, vectors, matrices

\newcommand{\justafunction}{\ensuremath{g}}
\newcommand{\justavector}{\ensuremath{v}}
\newcommand{\justamatrix}{\ensuremath{M}}
% used when we do not want to enforce the interpretation of a parameter space etc.

% probability things

\newcommand{\empprob}{\ensuremath{\mathbb P}}

\newcommand{\prob}{\ensuremath P}
\newcommand{\pd}{\ensuremath P}
\newcommand{\densityf}{\ensuremath{f}}

\newcommand{\Exp}{\ensuremath{\text{\rm E}}}
\newcommand{\cov}{\ensuremath{\text{\rm cov}}}
\newcommand{\var}{\ensuremath{\text{\rm var}}}
\newcommand{\noiseterm}{\ensuremath{Z}}

\newcommand{\expprior}{\ensuremath{q}}



%models 

\newcommand{\Bernoulli}{\ensuremath{\mathcal{B}}}
\newcommand{\BernoulliN}[1]{\ensuremath{{\mathcal{B}}^{(#1)}}}
\newcommand{\fakemarkov}{\ensuremath{\dddot{\Bernoulli}}}
\newcommand{\M}{\ensuremath {{\cal M}}}
\newcommand{\MN}[1]{\ensuremath {{\cal M}^{(#1)}}}
  %these are 'candidate hypotheses'

% Fisher inf stuff

\newcommand{\observedmatrix}{\ensuremath J}
%H already used for entropy
\newcommand{\fishermatrix}{\ensuremath I}
\newcommand{\curvelength}[1]{\ensuremath{\int_{#1} \fisherdens d\theta }}
\newcommand{\fisherdens}{\ensuremath{\sqrt{\det \fishermatrix(\theta)}}}
\newcommand{\fishervolume}{\ensuremath{V_{\text{d}}}}


% CHAPTER 3 

\newcommand{\level}{\mbox{\sc level}}
\newcommand{\descendantset}{\mbox{\sc d}}
\newcommand{\precision}{\ensuremath{d}}


\newcommand{\kl}{\mbox{$D$}}
\newcommand{\entropy}{{\ensuremath{\text{\rm H}}}}

% CHAPTER 4 


% CHAPTER 6, 7

\newcommand{\jp}{\ensuremath{w_{\text{Jef}}}}
\newcommand{\Lref}{\ensuremath{\mathcal{L}_{\text{ref}}}}
\newcommand{\pmodel}{\ensuremath{\theta}}
\newcommand{\prior}{\ensuremath{w}}
\newcommand{\discreteprior}{\ensuremath{W}}
\newcommand{\decision}{\ensuremath{\delta}}
\newcommand{\decisionspace}{\ensuremath{\Delta}}
\newcommand{\loss}{\ensuremath{\text{\sc loss}}}
\newcommand{\emptysequence}{\ensuremath{\text{\sc doen}}}
\newcommand{\realprob}{\ensuremath{\text{\sc doen}}}
\newcommand{\popt}{\ensuremath{\text{\sc doen}}}
\newcommand{\opthypothesis}{\ensuremath{\text{\sc doen}}}
%MOET ANDERS!




\newcommand{\volume}{\ensuremath{V_{\text{p}}}}
\newcommand{\Mdisc}{\ensuremath{\ddot{\mathcal M}}}
\newcommand{\probset}{\ensuremath{{\mathcal P}}}
\newcommand{\complexity}{\ensuremath{\text{\bf COMP}}}
\newcommand{\rcomplexity}{\ensuremath{\text{\bf RCOMP}}}
\newcommand{\typset}{\ensuremath{{\mathcal A}}}

%----------------------------------------------------------
% POST chapter 7

%MML

\newcommand{\wftwopartlength}{\ensuremath{L_{\ensuremath{\text{mml-wf}}}}}
\newcommand{\mmlplength}{\ensuremath{L_{\ensuremath{\text{mml-p}}}}}

%MaxEnt
\newcommand{\constraint}{\ensuremath{\mathcal C}}
\newcommand{\constraintdataset}{\ensuremath {{\mathbf C}^n}}
\newcommand{\entropified}[1]{\ensuremath{{\langle {#1} \rangle}}}
\newcommand{\range}{\ensuremath \mathbf U}
\newcommand{\expval}{\ensuremath t}
\newcommand{\mep}{\ensuremath{\prob_{me}}}
\newcommand{\mept}{\ensuremath{\prob_{me,\phi}(\cdot | t)}}
\newcommand{\freqdataset}{\ensuremath {{\mathbf G}^n}}
\newcommand{\freqdatasetn}[1]{\ensuremath {{\mathbf G}^{#1}}}
\newcommand{\constraintprobset}{\ensuremath {{\mathbf M}}}
\newcommand{\constraintdatasetn}[1]{\ensuremath {{\mathbf C}^{#1}}}
\newcommand{\empiricalconstraint}{\ensuremath {{\cal C}_{ e}}}
\newcommand{\average}[2]{\ensuremath \overline{#1}^{#2}}

% Unclear wether needed

%\newcommand{\maxnumclass}{\ensuremath K}
%\newcommand{\numcomps}{\ensuremath m}
%\newcommand{\numdimensions}{\ensuremath k}
%\newcommand{\traindata}{\ensuremath{D}}
\newcommand{\lagrange}{\ensuremath \beta}

% priors

%\newcommand{\jprior}{\ensuremath{\pi}}

%old

%\index{symbols}{zzz@$\tilde{c}$ where $c \in \{
%\pmodel,\lagrange,\hypothesis,\sigma \}$: model that minimizes expected error}
%\index{symbols}{zzz@$\hat{c}$ where $c \in \{
%\pmodel,\lagrange,\hypothesis,\sigma \}$: model that minimizes
%empirical error/maximizes likelihood}
%\index{symbols}{zzz@${c}_{mdl}$ where $c \in \{
%\pmodel,\lagrange,\hypothesis,\sigma \}$: model that minimizes
%two-part codelength}
%\index{symbols}{zzz@$\ddot{c}$ where $c \in \{
%\pmodel,\lagrange,\hypothesis \}$: (unspecified) estimator}
%\index{symbols}{zzz@$\breve{c}$ where $c \in \{
%\pmodel,\lagrange,\hypothesis \}$: Bayesian MAP estimator}
%\index{symbols}{zzz@$\bar{c}$ where $c \in \{
%\pmodel,\lagrange,\hypothesis \}$: mean of Bayesian posterior}
%\index{symbols}{zzz@$c^*$ where $c \in \{
%\pmodel,\lagrange,\hypothesis \}$: `true' model generating the data}

%\newcommand{\convergesatrate}{\ensuremath{\lesssim}}

